A Metaheuristic Algorithm for Large Maximum Weight Independent Set Problems

Motivated by a real-world vehicle routing application, we consider the maximum-weight independent set problem: Given a node-weighted graph, find a set of independent (mutually nonadjacent) nodes whose node-weight sum is maximum. Some of the graphs airsing in this application are large, having hundreds of thousands of nodes and hundreds of millions of edges. To solve instances of this size, we develop a new local search algorithm, which is a metaheuristic in the greedy randomized adaptive search (GRASP) framework. This algorithm, which we call METAMIS, uses a wider range of simple local search operations than previously described in the literature. We introduce data structures that make these operations efficient. A new variant of path-relinking is introduced to escape local optima and so is a new alternating augmenting-path local search move that improves algorithm performance. We compare an implementation of our algorithm with a state-of-the-art openly available code on public benchmark sets, including some large instances with hundreds of millions of vertices. Our algorithm is, in general, competitive and outperforms this openly available code on large vehicle routing instances. We hope that our results will lead to even better MWIS algorithms.

==> s_LP.tex <==
\section{Using LP Relaxation to Guild Local Search}
Recall that for graphs arising in our vehicle routing application,
we have additional clique information and can get a strong LP relaxation
solution.
This solution assigns each vertex a value in $[0,1]$
We use these values to guide the local search in Algorithm~\ref{alg:localsearch}.
When performing a random perturbation in Algorithm~\ref{alg:localsearch}, we add the vertex representing route $r$ to the solution with probability proportional to $x_r + \epsilon$. Here $\epsilon$ is a positive value (currently set to $\epsilon = 0.05$) that ensures that each vertex can be picked, even if $x_r = 0$.
This guides the local search by biasing route selection toward routes with higher fractional relaxed solution value.
The idea is that a route with a high value in the relaxed solution is more likely to be part of a good solution for the MWIS.
Using prefix sums we can pick a random route in time $\mathcal{O}(\log{|V|})$:
We draw a random floating-point number $z \in [0,\sum_{r \in R} x_r)$ and use binary search on the prefix sum array to pick a vertex such that the sum up to but excluding the vertex is less than $z$, and the sum up to and including the vertex is greater or equal to $z$.



==> s_app.tex <==
\section{\textcolor{red}{Motivating Application}}\label{s_app}
\textcolor{red}{
\note{RED TEXT REMOVED}
Although our algorithm is a general-purpose heuristic, our motivation
comes from long-haul vehicle routing (VR) 
\citep{DonGolNoeParResSpa21a,DonGolNoeParResSpa21b}, 
and a variant of our algorithm
takes advantage of the application-specific structure.}

\textcolor{red}{
To gain intuition into the application, consider a stochastic heuristic for
the problem that usually produces different solutions for different
pseudo-random generator seeds.
A well-known multi-start technique runs multiple {instantiations}
of the heuristic
in parallel and selects the best of the resulting solutions.
We want to do even better, i.e., use these multiple solutions to 
build a solution that
is better than the best of the input ones.
This is not always possible, e.g., if the best input solution is optimal.
However, in our application the technique usually succeeds.
}

\textcolor{red}{
A solution is a collection of routes.
Each {\em route} consists of a driver and a set of loads assigned to the driver.
A subset of routes is {\em feasible} if no two routes in the subset share
a driver or a load.
Note that we do not require a solution to cover all loads.
Each route {has} a weight, i.e., the benefit we get 
if we include the route in a solution.
The objective function is the sum of route weights.
The problem is to find a feasible solution of the maximum total weight.}

\textcolor{red}{
To state this problem as {an} MWIS, we build a {\em conflict graph} as follows.
Nodes of the graph correspond to routes and weights correspond to route
weights.
We connect two nodes by an edge if the corresponding routes have a conflict:
they share a driver or a load.
One can easily see that the maximum independent set in the conflict graph
corresponds to the optimal subset of routes in the original problem.
Some of the MWIS problems we get are large and have close to
$900$ thousand nodes and $400$ million edges.}

\textcolor{red}{
Note that in our application, we have a good initial solution,
the best of the solutions we combine.
We use this solution to warm-start our MWIS algorithm.
Our experiments show how much the warm-start helps.
}

\textcolor{red}{
For a fixed load (or driver), nodes corresponding to the routes
containing the load (driver) form a clique: every pair of such nodes is
connected.
This allows us to use the clique IP formulation of the problem introduced in
Section~\ref{s_intro} and solve the LP relaxation of the problem.
A variant of our algorithm uses the relaxed solution
to improve local search performance.}

\textcolor{red}{
Note that we do not have information
about all cliques in the graph; the next paragraph has an example.
This leads to a somewhat weaker IP formulation.
However, the relaxed solutions we get are good enough to improve
local search performance.}

\textcolor{red}{
The following example shows that we may not get all cliques.
Consider routes with three drivers,
$x$, $y$, and $z$, and three loads, $A$, $B$, and $C$.
Suppose we have the following three routes:
%\note{AVG: Changed this paragraph, please check}
\begin{enumerate}
\item
  $(x, A, B)$
\item
  $(y, A, C)$
\item
  $(z, B, C)$
  \end{enumerate}
These routes have no driver conflicts.
Each load appears in two routes and induces a 2-clique in the graph.
However, the graph itself is a 3-clique that does not correspond to any
clique induced by a driver or a load.}



==> s_blending.tex <==
%\section{Solution Blending}




\section{GRASP with solution-blending}
\label{s_gpr}

Path-relinking adds a long-term
memory mechanism to GRASP heuristics.
GRASP with path-relinking \citep{LagMar99a}
implements long-term memory by maintaining an
elite set of diverse high-quality solutions found during the search.
At each iteration, path-relinking is applied
between the solution found at the end of the local search phase and
a randomly-selected solution from the elite set.
The solution resulting from path-relinking is a candidate for inclusion in the
elite set.
A survey of path-relinking can be found in \citet{RibRes12a}.
See also \citet{ResRib16a} for an in-depth discussion of GRASP with
path-relinking.

%Similarly to path-relinking the solution blending technique add a long-term memory mechanism to GRASP heuristics.

In this paper, we introduce a different technique for combining two solution, that we call solution-blending.
Solution-blending is similar to path-relinking, but explores the two solutions
in a different way.

\subsection{Solution-blending for maximum-weight independent set}
\label{ss_pr}

Good solutions for a combinatorial optimization problem often share 
a significant
portion of their attributes. 
An example of such attributes in the maximum-weight independent set problem
are the nodes that make up a solution $S$.

Given two locally optimal solutions, we wish to explore different combinations
of these solutions.
The goal is to find solutions that can lead to better local optima. 
The motivation behind this approach is that some local optima solutions might contain good sub-solution for some part of the graph,
while poor sub-solution for the other part.
%After exploring several combinations of two solutions we choose the one with the greatest value as a starting point for our next
Note that solution-blending is also a way of escaping a stable local optima.

Given two solution $S_1, S_2$, we \emph{force} a node $v\in S_2$ into $S_1$ by inserting $v$ into $S_1$ and removing all of it's neighbors in $G$ from $S_1$; if $v$ is already in $S_1$, we do nothing.
The solution-blending procedure takes two solutions $S_1, S_2$ to the MWIS problem as an input..
First, the procedure makes a copies ${S_i}'$ of $S_i$ ($i = 1, 2$), which it uses to maintain modified versions of the solutions.
We process the nodes in $S' = S_1 \triangle S_2$ in a random order, where $\triangle$ the symmetric difference operator over sets of elements, and for each vertex $v \in S'$ we force $v$ into $S'_i$.
In addition, after we force a vertex into a solution, we make the solution maximal by inserting randomly vertices with no neighbors in the solutions. 


\begin{algorithm}[t!]
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{Two solutions $S_1, S_2$ to the MWIS problem on graph $G$}
	\Output{A new solution to the MWIS problem}
	\BlankLine
	$S'_{1} \leftarrow S_1$; $S'_{2} \leftarrow S_2$; $counter_1 \leftarrow 0$;$counter_2 \leftarrow 0$
	
	$S_{best} \leftarrow \emptyset$
	
	$SymmDiff \leftarrow S_1 \triangle S_2$
	
	\For{\textit{all} $v \in SymmDiff$ \textit{in a random order}}{
		
		\If{$v \notin S'_1$}{
			$S'_1 \leftarrow S'_1 \setminus N_G(v)$;
			$S'_1 \leftarrow S'_1 \cup \{v\}$;
			$counter_1 \leftarrow counter_1+1$
			
			Make $S'_1$ maximal
			
			\lIf{$counter_1 \geq \log(|S_1|) \textit{ and } \weight{S'_1}>\weight{S_{best}}$}{$S_{best} \leftarrow S'_1$}
		}
		
		\If{$v \notin S'_2$}{
			$S'_2 \leftarrow S'_2 \setminus N_G(v)$;
			$S'_2 \leftarrow S'_2 \cup \{v\}$; 
			$counter_2 \leftarrow counter_2+1$
			
			Make $S'_2$ maximal
			
			\lIf{$counter_1 \geq \log(|S_2|) \textit{ and } \weight{S'_2}>\weight{S_{best}}$}{$S_{best} \leftarrow S'_2$}
		}
	}
	Return $S_{best}$
	
	\caption{$\solutionblending(S_{1}, S_{2})$}
	\label{alg:solution-blending}
\end{algorithm}

Unlike path-relinking, solution-blending does not transform the first solution into the second and vice versa.
Instead, it explores different combination of the two solutions at different parts of the graph.The intuition is as follows.
First, we explore the general observation that the shared parts of two good solutions are often good.
Second, if there exists a part of the graph for which one solution contains a better sub-solution, then there is a probability with which parts of this sub-solution will be transferred into the second solution.

Notice that the description above is unidirectional, in the sense that is starts with solution $S_1$ and blends it with solution $S_2$. 
However, we can apply the same idea starting from $S_2$ and blending it with $S_1$.
Moreover, we ignore the solutions produced by very few
($\log(|S_i|)$ in out implementation) forced insertions around the two initial solutions, as these are likely to be in the neighborhood of the stable local optima solutions, and hence will lead to the same local optima after applying local search.
Algorithm \ref{alg:solution-blending} contains the pseudocode of the solution-blending procedure for the MWIS problem.
We also implemented path-relinking, but it gave worse results.

%Define an undirected graph $\mathcal{G} = (\mathcal{F}, \mathcal{M})$ associated with the search space of the maximum-weight independent set problem,  where the nodes in $\mathcal{F}$ correspond to feasible solutions and  the edges in $\mathcal{M}$ correspond to moves in some neighborhood structure $\mathcal{N}$ of the problem,  i.e. $(S, S') \in \mathcal{M}$ if and only if solutions $S \in \mathcal{F}$, $S' \in \mathcal{F}$, $S' \in \mathcal{N}(S)$, and $S \in \mathcal{N}(S')$.

%Paths between a pair of nodes $S$ and $T$ in the search space graph $\mathcal{G} = (\mathcal{F}, \mathcal{M})$ traverse other solutions that share attributes contained in $S$ and $T$. 
%The underlying assumption of path-relinking is that undiscovered high-quality solutions can be found by exploring paths connecting previously found high-quality elite solutions.  To generate the desired paths, it is only necessary to select moves that upon starting from an initiating solution $S$ progressively introduce attributes contributed by a guiding  solution $T$. 
% In the case of the maximum-weight independent set problem, the introduction of an attribute can be either the introduction in $S$ of a node in $T$ which is not in $S$ or removal from $S$ of a node in $S$ but not in $T$.
% The construction of such paths in the search space graph characteristically connects previous  points in ways not achieved in the previous search history  \citep{Glo99a},  often leading to better local optima.



\begin{figure}
\centering
\includegraphics[width=0.65\textwidth]{PRMWIS.eps}
\caption{Example of a path in the solution space between two solutions
$S$ (initial solution) and $T$ (guiding solution).  
A solution which is better than both $S$ and $T$ is found 
in the interior of the path.}
\label{f_PRMWIS}
\end{figure}

\note{NP: to change the example}
The example in Figure~\ref{f_PRMWIS} illustrates a path between two solutions,
the initial solution $S$ and the guiding solution $T$, 
having weights 11 and 14, respectively.
Starting at $S_0=S$, the first step in the path is generated 
by first removing from $S_0$ 
the node of
weight 4 (note that this node is not part of the guiding solution $T$).  
This results in a new solution, which we call $S_1$ with weight 7.
By adding the node of weight 9 into $S_1$ (note that this node is
present in the guiding solution $T$), 
we get a new solution, $S_2$, of weight 16. 
Removing from $S_2$ the node of weight 7 (note that that node is not
part of of the guiding solution $T$) leads us to 
a new solution $S_3$ of weight 9.
Finally, by adding to $S_3$ the node of weight 5, leads us to the guiding
solution $T$.
The best solution found in this path is $S_2$ of weight 16.
This solution turns out to be the global maximum for this problem instance.

%\begin{figure}[h]
%\begin{center}
%\framebox{
%\begin{minipage}[t]{20.8cm}
%\begin{tabbing}
%xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\= \kill
%{\bf begin} PATH-RELINKING$(S,T)$ \\
%1   \>${\Gamma^+} \gets (S \cup T) \setminus S$;\\
%2   \>${\Gamma^-} \gets (S \cup T) \setminus T$;\\
%3   \>${S^*} \gets \mathrm{argmax}\{ w(S), w(T) \}$;\\
%4   \>${w^*} \gets \max \{ w(S), w(T) \}$;\\
%5   \>{\bf while} $\Gamma^+ \cup \Gamma^- \not= \varnothing$ {\bf do}\\
%6   \> \>$v^* \gets \mathrm{argmax} \{ w(S \cup \{ v \}) \;:\; v \in \Gamma^+ \}$;\\
%7   \> \>$u^* \gets \mathrm{argmax} \{ w(S \setminus \{ u \}) \;:\; u \in \Gamma^- \}$;\\
%8   \> \>{\bf if} $w(S \cup \{ v^* \}) > w(S \setminus \{ u^* \})$ {\bf then}\\
%9   \> \> \>$S \gets S \cup \{v^*\}$;\\
%10   \> \> \>$\Gamma^+ \gets \Gamma^+ \setminus \{v^*\}$;\\
%11   \> \>{\bf else}\\
%12   \> \> \>$S \gets S \setminus \{u^*\}$;\\
%13   \> \> \>$\Gamma^- \gets \Gamma^- \setminus \{u^*\}$;\\
%14   \> \>{\bf end-if};\\
%15  \> \>{\bf if} $w(S) > w^*$ {\bf then}\\
%16  \> \> \>$S^* \gets S$;\\
%17  \> \> \>$w^* \gets w(S^*)$;\\
%18   \> \>{\bf end-if};\\
%19 \>{\bf end-while};\\
%20   \>$S^* \gets \textrm{LOCAL-SEARCH}(S^*)$;\\
%21 \>{\bf return} $S^*$;\\
%{\bf end} PATH-RELINKING.
%\end{tabbing}
%\end{minipage}
%}
%\end{center}
%\caption{Pseudo-code of a path-relinking algorithm
%for maximum-weight independent set.}
%\label{f_pr}
%\end{figure}

%Figure~\ref{f_pr} shows pseudo-code for a path-relinking algorithm
%that connects two solutions, $S$ and $T$, of the maximum-weight independent set 
%problem, starting from $S$ and using $T$ as a guide.
%A path in the solution space graph is constructed from $S$ to $T$.
%In that path, the algorithm searches for the best solution and returns a local optima obtained by applying local search to the best solution.  Lines~1 and~2 compute, respectively, that sets of nodes to be added to $S$ and to be removed from $S$ in the process of generating a path from $S$ to $T$. These sets are, respectively, $\Gamma^+$ and $\Gamma^-$. Lines~3 and~4 initialize, respectively, the best solution $S^*$ in the path and its weight $w^*$. The path is constructed in the loop from line~5 to line~19. To simplify the description of the algorithm we do not consider the case where only one of the sets  $\Gamma^+$ and $\Gamma^-$ is empty. This needs to be considered in an implementation of the algorithm. Lines~6 and~7 determine the best nodes to add to $S$ and to remove from $S$. These nodes are, respectively, $v^*$ and $u^*$. The greedy move is carried out in lines~8 to~14 where either set $\Gamma^+$ or set $\Gamma^-$ is updated accordingly. In lines~15 to~18, the best solution and its weight are updated if necessary. Finally, in line~20 a local search is applied, starting from the best solution found $S^*$ and the local maximum returned by the local search is returned as the path-relinking solution.

%\subsection{Truncated mixed path-relinking}
%\label{ss_tmpr}

%The solution-blending operator described in Section~\ref{ss_pr} is unidirectional in the sense that the roles of $S$ and $T$, either initial or guiding solutions, must be specified.
%Usually one assigns the initial solution $S$ to be the best of the two and the guiding solution $T$ to be the  \textcolor{black}{worse}.
% This way path-relinking explores more intensely the neighborhood around $S$.
% One drawback of unidirectional path-relinking is that the search is confined to exploration around only one of the solutions to be relinked.
% One way to get around this is to do \textit{bidirectional} path-relinking, where one applies the operator from $S$ to $T$ and then from $T$ to $S$.
%Bidirectional path-relinking explores the two neighborhoods at the expense of approximately twice the computation time.
%Mixed path-relinking explores both neighborhoods without taking as long as `bidirectional path-relinking.

%In \textit{mixed} path-relinking, $S$ and $T$ are  initially assigned the roles of initial and guiding solutions. After each iteration, the roles are interchanged, i.e. the current solution $S$ becomes $T$ and the current $T$ becomes $S$. Again, attributes of $T$ not present in $S$ are introduced in $S$.

%Experience with the use of path-relinking  has  shown (see, e.g. \citet{ResMarGalDua10a}) that improvements are most likely to be encountered near the initial set of solutions.
%To capitalize on this observation, \textit{truncated} path-relinking limits its exploration to a few moves from each extreme. We use the same idea in our implementation by limiting the exploration to a few forced insertions away from each of the initial solutions. 


In our implementation of GRASP with solution-blending for the 
maximum-weight independent set problem, we use solution-blending with
a truncated bidirectional search:
we modify both $S-1'$ and $S_2'$, but stop the blending loop after a fixed
number of iterations.\note{AVG: is this corect?}

\subsection{Hybridization of solution-blending and GRASP
for maximum-weight independent set}
\label{ss_gpr}

We use the elite set to combine GRASP and solution-blending.
An \textit{elite set} is a diverse, limited-size set
of good solutions found by the search over time.
The elite set a memory structure in GRASP.
An elite set $\mathcal{E}$ has to support three operations.
First, given a solution $S$, we need to be able to determine
whether $S$ will be added to $\mathcal{E}$. 
Second, if $\mathcal{E}$ is full and we insert solution $S$ into
$\mathcal{E}$, we need to be able to determine which solution 
$S' \in \mathcal{E}$ will be replaced by $S$.
Finally, we need to select an element from $\mathcal{E}$ at random.


\begin{algorithm}[t!]
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{A weighted graph and time limit $t_{limit}$ \xspace}
	\Output{An independent set}
	\BlankLine
	$S_{best} \leftarrow \emptyset; \mathcal{E}\leftarrow \emptyset$; 
	
	\While{time did not exceed $t_{limit}$}{
		$S_{greedy} \leftarrow \graspconstruction()$
		
		$S_{elite} \leftarrow \arg \max_{S\in \mathcal{E}} \{|S \triangle S_{greedy}|\}$
		
		$S_{blended} \leftarrow \solutionblending(S_{greedy}, S_{elite})$
		
		$S_{LS} \leftarrow \perturbLS(S_{blended})$
		
		\lIf{$\weight{S_{SLS}}>\weight{S_{best}}$}{
			$S_{best} \leftarrow S_{LS}$
		}
		
		\uIf{$\mathcal{E}$ is not full and $S_{SLS} \notin \mathcal{E}$}{
			add $S_{SLS}$ to $\mathcal{E}$
		}
		\ElseIf{$\weight{S_{SLS}} \geq \arg \min_{S\in \mathcal{E}}\{\weight{S}\}$}{
			$S_{out} \leftarrow \arg \min_{S\in \mathcal{E}, \weight{S} \leq \weight{S_{SLS}}} \{|S \triangle S_{SLS}|\}$
			
			$\mathcal{E} = \mathcal{E}\cup S_{SLS}$
			
			$\mathcal{E} = \mathcal{E}\setminus S_{out}$
		}
	}
	Return $\arg \max_{S\in \mathcal{E}}\{\weight{S}\}$
	\caption{GRASP with solution-blending for MWIS}
	\label{alg:grasp-with-solution-blending}
\end{algorithm}

%\begin{figure}[h]
%\begin{center}
%\framebox{
%\begin{minipage}[t]{20.8cm}
%\begin{tabbing}
%xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\= \kill
%{\bf begin} GRASP+PR \\
%1   \>${f^*} \gets -\infty$;\\
%2   \>$i \gets 1$;\\
%3   \>$\mathcal{E} \gets \varnothing$;\\
%4   \>{\bf while} stopping criterion not satisfied {\bf do}\\
%5   \> \>$S^i \gets \textrm{GREEDY-RANDOMIZED-CONSTRUCTION}$;\\
%6   \> \>$S^i \gets \textrm{LOCAL-SEARCH}(S^i)$;\\
%7   \> \>{\bf if} $\mathcal{E}$ is empty {\bf then}\\
%8   \> \> \>$\textrm{INSERT-INTO-ELITE}(S^i, \mathcal{E})$;\\
%9   \> \>{\bf else}\\
%10   \> \> \>$S' \gets \textrm{SELECT-FROM-ELITE}(S^i, \mathcal{E})$;\\
%11   \> \> \>$S^i \gets \textrm{PATH-RELINKING}(S^i, S')$;\\
%12   \> \> \>$\textrm{UPDATE-ELITE}(S^i, \mathcal{E})$;\\
%13   \> \>{\bf end-if};\\
%14   \> \>{\bf if} $f(S^i) > f^*$ {\bf then}\\
%15   \> \> \>$S^* \gets S^i$;\\
%16   \> \> \>$f^* \gets f(S^i)$;\\
%17   \> \>{\bf end-if};\\
%18  \> \>$i \gets i+1$;\\
%19 \>{\bf end-while};\\
%20 \>{\bf return} $S^*$;\\
%{\bf end} GRASP+PR.
%\end{tabbing}
%\end{minipage}
%}
%\end{center}
%\caption{Pseudo-code of a basic GRASP with path-relinking
%heuristic for maximization.}
%\label{f_grasp-pr_max}
%\end{figure}

Algorithm ~\ref{alg:grasp-with-solution-blending} 
shows pseudo-code for a GRASP with a solution-blending heuristic for
a maximization problem.
This heuristic visits a sequence of local maxima
$S_1, S_2, \ldots, S_q$, and returns the
best solution visited, $S_{best}$.
Initializations of the best solution and the elite set $\mathcal{E}$ are made in Line~1. 
The limit on the size of the elite set is not spelled out explicitly in the pseudocode.
GRASP with solution-blending iterations are carried out in the
loop in Lines~2 to~13.
Line~3 produces a solution $S_{greedy}$ through
randomized greedy construction.
In Line~4, the algorithm selects from the elite set the solution $S_{elite}$
which is most different from $S_{greedy}$ (i.e., the one that maximizes the cardinality of the symmetric difference with $S_{greedy}$).
Line~5 executes solution-blending between $S_{elite}$ and $S_{greedy}$ and produces a solution $S_{blended}$. 
The algorithm then proceeds with identifying a stable local optimum solution $S_{SLS}$, using the algorithm from Section \ref{sec:stable-local-search}, starting from $S_{blended}$.

After we obtain a stable locally optimal solution $S_{SLS}$, the elite set may have to be updated 
There are two cases.
\begin{enumerate}
\item If $\mathcal{E}$ is not full, then $S_{SLS}$ is added to the elite set if it is not already in the set.
\item If $\mathcal{E}$ is full, then $S_{SLS}$ is added to the elite set only if $w(S_{SLS}) \geq \arg \min_{S\in \mathcal{E}}\{\weight{S}\}$. If $S_{SLS}$ is added to the elite set, then it must replace some solution $S_{out}$ currently in the elite set. Among all elite set solutions weighing at most as $S_{SLS}$, replace the one most similar to $S_{SLS}$, i.e.
\begin{displaymath}
S_{out} \leftarrow \arg \min_{S\in \mathcal{E}, \weight{S} \leq \weight{S_{SLS}}} \{|S \triangle S_{SLS}|\}
\end{displaymath}
Notice that if $\mathcal{E}$ contains a solution identical to $S_{SLS}$, then this solution is replaced by $S_{SLS}$, avoiding multiple identical solutions in the elite set.
\end{enumerate}
%If a new best solution is found, then it and its weight are saved in lines~15 and~16. The iteration counter is updated in line~18 and the best solution found is returned in line~20.
After reaching a maximum time limit, the algorithm returns the best solution from the elite set.

%Following the stable local search, if the elite set  $\mathcal{E}$  is not full, the solution $S_{SLS}$ is added to $\mathcal{E}$ in line~8.
%Otherwise, if $S_{SLS}$ is better than the worse solution in $\mathcal{E}$, in Lines~10~-~13 the algorithm adds $S_{SLS}$ into $\mathcal{E}$  and removes from it the solution $S_{out}$ such that $w(S_{out}) < w(S_{SLS})$ and such that it minimizes the cardinality of the symmetric difference with $S_{SLS}$.

%Let $\mathcal{I}(S)$ be a 0~-~1 indicator vector associated with solution $S$ such that $\mathcal{I}(S)_j=1$ if and only if node $v_j \in S$, for $j=1,2,\ldots,|V|$.
%Let the \textit{Hamming distance} between any two solutions $S$ and $T$ be  $$\mathcal{H}(S, T) = \sum_{j=1}^{|V|} | \mathcal{I}(S)_j - \mathcal{I}(T)_j |.$$
%Given the locally maximum solution $S^i$ produced in line~6, $S'$ is selected at random from solutions $S \in \mathcal{E}$ with probability proportional to   $\mathcal{H}(S^i, S)$, i.e. the selection favors solutions $S \in \mathcal{E}$  that differ more from $S^i$ than those that are similar to $S^i$.
%This selection method leads to longer paths in  the path-relinking operation in line~11.

%Once a local maximum $S^i$ is produced by path-relinking in line~11,  the elite set may have to be updated in line~12. 
%There are two cases.
%\begin{enumerate}
%\item If $\mathcal{E}$ is not full, then $S^i$ is added to the elite set only if it differs from all solutions in the set, i.e. only if there is no $S \in \mathcal{E}$ for which  $\mathcal{H}(S^i, S) = 0$.
%\item If $\mathcal{E}$ is full, then $S^i$ is added to the elite set only if $w(S^i) > w_{\min}$, where  $$w_{\min} = \min \{w(S) \;|\; S \in \mathcal{E} \},$$ and $S^i$ differs from all solutions in the set. If $S^i$ is added to the elite set, then it must replace some solution $S^+$ currently in the elite set. Among all elite set solutions weighing less than $S^i$, replace the one most similar to $S^i$, i.e.
%\begin{displaymath}
%S^+ = \mathrm{argmin} \{ \mathcal{H}(S^i,S), \forall S \in \mathcal{E} \;|\; w(S) < w(S^i) \}
%\end{displaymath}
%is chosen to be removed from the elite set.
%\end{enumerate}
%If a new best solution is found, then it and its weight 
%are saved in lines~15 and~16. The iteration counter is updated in line~18 and the best solution found is returned in line~20.

%\subsection{Evolutionary path-relinking}

%At the conclusion of GRASP+PR, we are left with an elite set $\mathcal{E}$.
%Evolutionary path-relinking \citep{ResWer04a,ResMarGalDua10a} is an intensification process on the elite set.
%It starts with the final elite set $\mathcal{E}$ after GRASP+PR as a starting point and marks all pairs of elite set solutions $\{S_1^1,S_1^2\}$, $\{S_2^1,S_2^2\}$, $\ldots$, as \textit{unlinked}, where $S_i^j \in \mathcal{E}$, for $j=1,2$ and $i=1,2,\ldots, \binom{|\mathcal{E}|}{2}$.
%Let $k=0$ and $\mathcal{E}_k = \mathcal{E}$.  
%While there exist $S_k^1 \in\mathcal{E}_k$ and $S_k^2 \in\mathcal{E}_k$ such that the pair $\{S_k^1,S_k^2\}$ is marked \textit{unlinked}, mark the pair \textit{linked} and let $T \gets  $ PATH-RELINKING$(S_k^1,S_k^2)$ and UPDATE-ELITE$(T,\mathcal{E}_k)$.
%Let the updated elite set be $\mathcal{E}_{k+1}$ and let $k \gets k+1$. If $T$ was accepted into $\mathcal{E}_k$, then mark all  pairs $\{T,S_k\}$ \textit{unlinked}, for all  $S_k \in \mathcal{E}_k \setminus \{T\}$.
%If all pairs of solutions in $\mathcal{E}_k$ are marked \textit{linked}, return the best solution in  $\mathcal{E}_k$ as the solution of evolutionary path-relinking.
%Line~20 of the pseudo-code in Figure~\ref{f_grasp-pr_max} becomes:

%\vspace*{15pt}
%\noindent
%\textbf{return} $S^* \gets $EVOLUTIONARY-PR$(\mathcal{E})$.



==> s_def.tex <==
\section{Definitions and Notation}
\label{s_def}

For the input graph $G = (V,E)$, let $n = |V|$ and $m = |E|$
be the number of vertices and edges, respectively.
For a vertex $v$, we denote the set of neighbors of $v$ by $N(v)$.


==> s_grasp.tex <==
\section{GRASP for maximum-weight independent set}
\label{s_grasp}

Our algorithm is based on GRASP, introduced by
\citet{FeoRes89a} in the context of the set covering problem.
\citet{FeoRes95a} generalizes GRASP as a metaheuristic for combinatorial optimization.
See also \citet{ResRib16a} for an in-depth discussion.
Let $U$ the universe of elements that are contained in solutions to the problem at hand.
Figure~\ref{f_grasp_max} gives GRASP pseudocode.
The function $f:2^U\rightarrow \mathbb{R}$ denotes the objective function.
GRASP uses a randomized greedy algorithm with multiple pseudorandom generator
seeds to compute feasible initial solutions $S^1, S^2, \ldots$.
For each initial solution, we run local search to compute a locally optimal solution.
GRASP returns the best of these solutions:
\begin{displaymath}
S^* = \mathrm{argmax} \{ f(S^i), i=1, 2,\ldots \}, 
\end{displaymath}

\begin{figure}[t!]
	\begin{center}
		\framebox{
			\begin{minipage}[t]{20.8cm}
				\begin{tabbing}
					xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\= \kill
					{\bf begin} GRASP \\
					1   \>${f^*} \gets -\infty$;\\
					2   \>$i \gets 1$;\\
					3   \>{\bf while} stopping criterion not satisfied {\bf do}\\
					4   \> \>$S^i \gets \textrm{GREEDY-RANDOMIZED-CONSTRUCTION}$;\\
					5   \> \>$S^i \gets \textrm{LOCAL-SEARCH}(S^i)$;\\
					6   \> \>{\bf if} $f(S^i) > f^*$ {\bf then}\\
					7   \> \> \>$S^* \gets S^i$;\\
					8   \> \> \>$f^* \gets f(S^i)$;\\
					9   \> \>{\bf end-if};\\
					10  \> \>$i \gets i+1$;\\
					11 \>{\bf end-while};\\
					12 \>{\bf return} $S^*$;\\
					{\bf end} GRASP.
				\end{tabbing}
			\end{minipage}
		}
	\end{center}
	\caption{Pseudo-code of a basic GRASP heuristic for maximization.}
	\label{f_grasp_max}
\end{figure}

\citet{FeoResSmi94a} applied GRASP to the maximum cardinality
independent set ({\em MCIS}) problem as follows.
Given a graph $G=(V,E)$, a feasible solution $S$ of the MCIS
problem is a set $S \subseteq V$ of pairwise nonadjacent nodes in $G$. 
Let $\mathrm{deg}_S (v)$ be the degree of node $v \in V$ with respect to $S$,
i.e. 
$\mathrm{deg}_S (v) = | \{ (v,u) \in E \;|\; u \in S \} |$. 
A solution $S$ is \emph{maximal} if and only if 
there is no node $v \in V \setminus S$ such that 
$\mathrm{deg}_S (v) = 0$.
If such node existed, it could be added to the solution, increasing its 
cardinality by one.
\citet{FeoResSmi94a} use 
a randomized greedy algorithm 
to build a maximal independent set, one node at a time.
Let $C \subseteq V$ be the set of admissible nodes, 
i.e. nodes that could be added to a non-maximal
solution $S$ without destroying its independence property. 
Initially $S = \varnothing$ and $C = V$.
At each iteration, we select a node $v \in C$ having the minimum
$\deg_C (v)$. Call this node $v^*$.
Add $v^*$ to $S$ and remove from $C$ all nodes adjacent to $v^*$ in $G$.
The procedure is repeated until $C = \varnothing$.

The above-described construction procedure does not consider weighted 
graphs, like in the problem we have on hand.
Consider the graph in Figure~\ref{2v3IS} where node weights are
indicated on each node.
This graph illustrates the case where a smaller cardinality 
independent set (Gray nodes) has
greater weight (16) than a larger cardinality set (black nodes) whose
weight is 13.
A greedy algorithm for the maximum-weight independent set ({\em MWIS}) problem also builds 
an independent set, one node at a time.
Initially $S = \varnothing$ and $C = V$.
At each iteration of this greedy algorithm,
select a node $v \in C$ having maximum
$w_v \div \deg_C (v)$ value. Call this node $v^*$.
Without loss of generality, we can assume $\deg_C (v)>0$, for all $v \in V$,
since isolated nodes $v$ can
be added to the independent set as long as $w_v \geq 0$.  
As before, 
add $v^*$ to $S$ and remove from $C$ all nodes adjacent to $v^*$ in $G$.
The procedure is repeated until $C = \varnothing$.

Applying the greedy algorithm to the graph in Figure~\ref{2v3IS}, however,
results in a sub-optimal solution since
the algorithm would first choose the node of weight 5 on the right, then
the node of weight 4 in the bottom, and finally one of the two remaining
nodes of weight 4, resulting in an independent set of weight 13.
This is why GRASP runs a greedy construction followed by a local search.
%One is local search.
%Another is randomization of the greedy algorithm.
Next, we describe the construction and the search.

\subsection{Randomized greedy construction}
\label{s_semigreedy}
One approach to randomize the greedy algorithm is,
instead of selecting
the node 
$v \in C$ having maximum
$w_v \div \deg_C (v)$ value, to select at random from a set of nodes
having large
$w_v \div \deg_C (v)$ values.
Suppose that in the construction of the independent set of the graph
in Figure~\ref{2v3IS}, we were to choose at random from the pair of nodes
having largest $w_v \div \deg_C (v)$ values.
In the initial iteration, those two nodes would be the one with weight 5, for
which 
$w_v \div \deg_C (v) = 5/1 = 5$ and the one with weight 9, where
$w_v \div \deg_C (v) = 9/3 = 3$.
If the node of weight~9 is randomly
selected, then the only remaining nodes in set $C$ are the
two nodes with weights~5 and~7.
Selecting at random the one with weight~7 results in the
globally optimal solution (gray nodes) of weight~16.

Algorithm~\ref{f_construct} shows the pseudocode for the greedy randomized
construction algorithm used in the GRASP for MWIS described in this paper.
The procedure takes as input a random real-valued parameter 
$\alpha \in \mathrm{random}(\beta,1)$, where $\beta \in [0,1]$ is a
fixed real-valued parameter, the graph $G=(V,E)$ and the node weights 
$w_v$, $\forall v \in V$, and outputs an independent set $S \subseteq V$ whose
weight is $\sum_{v \in S} w_v$.



\begin{algorithm}[t!]
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{A weighted graph, and a value $\alpha$\xspace}
	\Output{An independent set $S$}
	\BlankLine
	$S \gets \varnothing$
	
	$C \gets V$
	
	\While{$C \not= \varnothing$}{
		$g_v \gets w_v \div \deg_C (v), \; \forall v \in C$
		
		$g^{\min} \gets \min\{g_v \;|\; v\in C\}$
		
		$g^{\max} \gets \max\{g_v \;|\; v\in C\}$
		
		$g^{+} \gets g^{\min} + \alpha (g^{\max} - g^{\min})$
		
		$\mathrm{RCL} \gets \{ v \in C \;|\; g_v \geq g^{+} \}$
		
		Select $v^* \in \mathrm{RCL}$ at random with probability proportional to $g_{v^*}$
		
		$S \gets S \cup \{ v^* \}$
		
		$\bar{C} \gets \{ v \in C \;|\; (v,v^*) \in E \}$
		
		$C \gets C \setminus \bar{C}$
	}
	
	{\bf return} $S$
	
	\caption{Greedy-Randomized-Construction}
	\label{f_construct}
\end{algorithm}

%\begin{figure}[h]
%\begin{center}
%\framebox{
%\begin{minipage}[t]{20.8cm}
%\begin{tabbing}
%xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\= \kill
%{\bf begin} GREEDY-RANDOMIZED-CONSTRUCTION$(\alpha,G=(V,E),w)$ \\
%1   \>$S \gets \varnothing$;\\
%2   \>$C \gets V$;\\
%3   \>{\bf while} $C \not= \varnothing$ {\bf do}\\
%4   \> \>$g_v \gets w_v \div \deg_C (v), \; \forall v \in C$;\\
%5   \> \>$g^{\min} \gets \min\{g_v \;|\; v\in C\}$;\\
%6   \> \>$g^{\max} \gets \max\{g_v \;|\; v\in C\}$;\\
%7   \> \>$g^{+} \gets g^{\min} + \alpha (g^{\max} - g^{\min})$;\\
%8   \> \>$\mathrm{RCL} \gets \{ v \in C \;|\; g_v \geq g^{+} \}$;\\
%9   \> \>Select $v^* \in \mathrm{RCL}$ at random;\\
%10   \> \>$S \gets S \cup \{ v^* \}$;\\
%11  \> \>$\bar{C} \gets \{ v \in C \;|\; (v,v^*) \in E \}$;\\
%12  \> \>$C \gets C \setminus \bar{C}$;\\
%13 \>{\bf end-while};\\
%14 \>{\bf return} $S$;\\
%{\bf end} GREEDY-RANDOMIZED-CONSTRUCTION.
%\end{tabbing}
%\end{minipage}
%}
%\end{center}
%\caption{Pseudo-code of a randomized greedy construction heuristic for
%maximum-weight independent set.}
%\label{f_construct}
%\end{figure}

The greedy randomized construction in Algorithm~\ref{f_construct}
builds an independent set $S$ one node at a time.
We initialize the current solution $S$ to an empty set and 
the candidate set $C$ to $V$.
The main loop of the construction algorithm runs until $C$ becomes empty.
At each iteration we evaluate
$g_v \gets w_v \div \deg_C (v), \; \forall v \in C$, compute the minimum
($g^{\min}$) and maximum ($g^{\max}$) values and a threshold value
$g^{+} \gets g^{\min} + \alpha (g^{\max} - g^{\min})$.
The latter defines the restricted candidate list (RCL),
consisting of all nodes $v$ for which the value of $g_v$ is at least $g^+$.
We select a node $v^*$ from RCL at random, with probability proportional
to the value $g_{v^*}$, and add $v^*$ to $S$.
Note that when $\alpha = 0$, the RCL will contain all nodes in $C$.
On the the other hand, when $\alpha = 1$, then the RCL will only contain
the nodes $v \in C$ for which $g_v = g^{\max}$, as in the deterministic greedy algorithm.
After we add $v^*$ to $S$, we update $C$ by removing from it all neighbors
of $v^*$ in $G$.
Once $C$ is empty, we return $S$.

Figure~\ref{f_construction} 
shows the
partial independent set (in red), and the set of candidate nodes
along with edges incident to two candidate nodes over 85 iterations
of a randomized greedy construction procedure for maximum
independent set on a graph with 303 nodes and 1114 edges. 
The size of the candidate set $C$ of nodes as well as the number of edges
incident to at least one candidate node over the randomized
greedy iterations are shown in the plot of Figure~\ref{f_construction-size}. 

\begin{figure}
	\centering
	%\begin{minipage}[t]{20.8cm}
	\begin{tabular}{| c | c | c | c|}
		\hline
		\includegraphics[width=0.20\textwidth]{0_neato.png}  &
		\includegraphics[width=0.20\textwidth]{20_neato.png}  &
		\includegraphics[width=0.20\textwidth]{30_neato.png}  &
		\includegraphics[width=0.20\textwidth]{40_neato.png} \\
		iteration 0 & iteration 20 & iteration 30 & iteration 40 \\
		\hline
		\includegraphics[width=0.20\textwidth]{50_neato.png} &
		\includegraphics[width=0.20\textwidth]{60_neato.png} &
		\includegraphics[width=0.20\textwidth]{70_neato.png} &
		\includegraphics[width=0.20\textwidth]{80_neato.png} \\
		iteration 50 & iteration 60 & iteration 70 & iteration 80 \\
		\hline
		\includegraphics[width=0.20\textwidth]{81_neato.png} &
		\includegraphics[width=0.20\textwidth]{82_neato.png} &
		\includegraphics[width=0.20\textwidth]{83_neato.png} &
		\includegraphics[width=0.20\textwidth]{84_neato.png} \\
		iteration 81 & iteration 82 & iteration 83 & iteration 84 \\
		\hline
	\end{tabular}
	%\end{minipage}
	\caption{Process of randomized greedy construction on a graph with 303 nodes and 1114 edges. Red nodes indicate
		partially constructed independent set.}
	\label{f_construction}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.65\textwidth]{construction-size.eps}
	\caption{Size of conflict graph during 
		process of randomized greedy construction on a graph with 303 nodes and 1114 edges.
	}
	\label{f_construction-size}
\end{figure}

\subsection{Variable neighborhood descent local search}
\label{sec:local-search}

\begin{algorithm}[t!]
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{A weighted graph, a time limit $t_{limit}$, an independent set $S$ \xspace}
	\Output{An independent set where no improving local move is possible}
	\BlankLine
	
	\While{time did not exceed $t_{limit}$}{
		$S \leftarrow S'$
		
		$S' \leftarrow \oneanymove(S)$
		
		\If{$S' = S$}{
			
			$S' \leftarrow \twoonemove(S)$
			
			\If{$S' = S$}{
				
				$S' \leftarrow \twotwomove(S)$
				
				\If{$S' = S$}{
					$S' \leftarrow \twothreemove(S)$
					
					\lIf{$S' = S$}{
						return $S$
					}
				}
			}
		}
		Make $S$ maximal
	}
	Return $S$
	\caption{$\LS(S)$}
	\label{f_local-search}
\end{algorithm}

Local search is a general heuristic approach used for solving optimization problems.
The local search algorithm starts with an arbitrary valid solution and iteratively swaps nodes or pairs of nodes in the solution with nodes or sets of nodes not in the solution.
In the example of Figure~\ref{2v3IS} starting with the independent set of
black nodes, consider first an improving swap where two nodes in the 
solution are replaced by one not in the solution.
Replacing the two black nodes of weight~4 with the gray node
of weight~9 improves the weight of the resulting independent set 
by one (to~14).
Then, by applying a swap where the node of weight~5 in the
solution is swapped with the one of weight~7, not in the solution, results in
the globally optimal solution (gray nodes) of weight~16.
\citet{FeoResSmi94a} used a swap-based local search for maximum cardinality
independent set problem in their GRASP heuristic.
\citet{AndResWer12a} introduced faster
local search algorithms for the maximum
cardinality independent set problem.

A (local search) {\em move} is a small modification of $S$.
Given a collection of moves and a solution $S$, the 
neighborhood $\mathcal{N}$ of $S$ is the set of solutions which one can obtain
from $S$ by applying a single move.
Local search starts with an initial solution $S^0$ and produces a sequence
of $q \geq 0$ improving solutions $S^1, S^2, \ldots, S^q$ such that
$S^{i+1} \in \mathcal{N}(S^i)$, for $i=0, 1, \ldots, q-1$.
The search terminates when there is no improving solution in the neighborhood
of $S$
In this case, we call $S$ a {\em locally optimal} solution.

Our local search algorithm uses the following moves:
\begin{itemize}
	\item \oneanymove: an improving move that adds a node $v\notin S$ to $S$ and removes any number of nodes $S_{out}\subset S$ from $S$, such that $\weight{v}>\weight{S_{out}}$.
	\item \twoonemove: an improving move that removes a node $v\in S$  from $S$ and adds two nodes $x,y \notin S$ in $S$, such that $\weight{\{x,y\}}>\weight{v}$.
	\item \twotwomove: an improving move that removes two nodes $u,v\in S$ from $S$ and adds two nodes $x,y \notin S$ to $S$, such that $\weight{\{x,y\}}>\weight{\{u,v\}}$.
	\item \twothreemove: an improving move that removes two nodes $u,v\in S$ from $S$ and adds three nodes $x,y,z \notin S$ to $S$, such that $\weight{\{x,y,z\}}>\weight{\{u,v\}}$.
\end{itemize}

%\begin{itemize}
%\item
%\textbf{1-1 swap:}
%Let $v \in S$, $u \in V \setminus S$, such that 
%$\deg_{S \setminus \{v\}}(u) = 0$ and $w_u > w_v$.
%If such nodes $u$ and $v$ exist, the improving
%solution $S'$ is obtained from $S$ by replacing $v$ in $S$
%with $u$.
%\item
%\textbf{1-2 swap:}
%Let $v \in S$, $u_1, u_2 \in V \setminus S$, such that 
%$(u_1,u_2) \not\in E$,
%$\deg_{S \setminus \{v\}}(u_1) = \deg_{S \setminus \{v\}}(u_2) = 0$ 
%and 
%$w_{u_1} + w_{u_2} > w_{v}$.
%If such nodes $u_1, u_2$, and $v$ exist, the improving solution $S'$
%is obtained from $S$ by replacing $v$ in $S$
%with $u_1$ and $u_2$.
%\item
%\textbf{2-1 swap:}
%Let $v_1, v_2 \in S$, $u \in V \setminus S$, such that 
%$\deg_{S \setminus (\{v_1\} \cup \{v_2\}) }(u) = 0$ and 
%$w_u > w_{v_1} + w_{v_2}$.
%If such nodes $u$, $v_1$, and $v_2$ exist, the improving
%solution $S'$ is obtained from $S$ by replacing $v_1$ and $v_2$ in $S$
%with $u$.
%\item
%\textbf{2-2 swap:}
%Let $v_1, v_2 \in S$, $u_1, u_2 \in V \setminus S$, such that 
%$(u_1,u_2) \not\in E$,
%$\deg_{S \setminus (\{v_1\}\cup\{v_2\})}(u_1) = \deg_{S \setminus (\{v_1\}\cup \{v_2\})}(u_2) = 0$ 
%and 
%$w_{u_1} + w_{u_2} > w_{v_1} + w_{v_2}$.
%If such nodes $u_1, u_2$, $v_1$, and $v_2$ exist, the improving
%solution $S'$ is obtained from $S$ by replacing $v_1$ and $v_2$ in $S$
%with $u_1$ and $u_2$.
%\end{itemize}
%If we assume $|V \setminus S| > |S|$, then the complexity of searching  the four neighborhoods above increases as we move from 1-1 swap to 1-2 swap to 2-1 swap to 2-2 swap. In such situations, a variable descent neighborhood local search provides a good balance between intensification depth and search complexity. The pseudo-code in Figure~\ref{f_local-search} shows how these local search neighborhoods can be combined.




%\begin{figure}[h]
%\begin{center}
%\framebox{
%\begin{minipage}[t]{20.8cm}
%\begin{tabbing}
%xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\=xxx\= \kill
%{\bf begin} LOCAL-SEARCH$(S,G=(V,E),w)$ \\
%1   \>{\bf while} $S$ is not a local maximum of the four neighborhoods {\bf do}\\
%2   \> \>$S' \gets \mbox{\tt 1-1-swap}(S)$;\\
%3   \> \>{\bf if} $w(S') > w(S)$ {\bf then}\\
%4   \> \> \>$S \gets S'$;\\
%5   \> \> \>{\bf continue};\\
%6   \> \>{\bf else}\\ 
%7   \> \> \>$S' \gets \mbox{\tt 1-2-swap}(S)$;\\
%8   \> \> \>{\bf if} $w(S') > w(S)$ {\bf then}\\
%9   \> \> \> \>$S \gets S'$;\\
%10   \> \> \> \>{\bf continue};\\
%11   \> \> \>{\bf else}\\ 
%12   \> \> \> \>$S' \gets \mbox{\tt 2-1-swap}(S)$;\\
%13   \> \> \> \>{\bf if} $w(S') > w(S)$ {\bf then}\\
%14   \> \> \> \> \>$S \gets S'$;\\
%15   \> \> \> \> \>{\bf continue};\\
%16   \> \> \> \>{\bf else}\\ 
%17   \> \> \> \> \>$S' \gets \mbox{\tt 2-2-swap}(S)$;\\
%18   \> \> \> \> \>{\bf if} $w(S') > w(S)$ {\bf then}\\
%19   \> \> \> \> \> \>$S \gets S'$;\\
%20   \> \> \> \> \> \>{\bf continue};\\
%21   \> \> \> \> \>{\bf end};\\ 
%22   \> \> \> \>{\bf end};\\ 
%23   \> \> \>{\bf end};\\ 
%24   \> \>{\bf end};\\ 
%25 \>{\bf end-while};\\
%26 \>{\bf return} $S$;\\
%{\bf end} LOCAL-SEARCH.
%\end{tabbing}
%\end{minipage}
%}
%\end{center}
%\caption{Pseudo-code of a variable descent local search for maximum-weight
%independent set using neighborhoods
%1-1 swap, 1-2 swap, 2-1 swap and 2-2 swap.}
%\label{f_local-search}
%\end{figure}

For efficiency, our local search algorithm,
outlined in Algorithm~\ref{f_local-search}, uses four different neighborhoods,
defined as follows:
%In Lines~3, 8, 12, and~18 of the pseudo-code, we represent  the weight $\sum_v \in S} w_v$ of a solution $S$ by $w(S)$.
$\mathcal{N}_1 =$ \oneanymove
$\mathcal{N}_2 =$ \twoonemove,
$\mathcal{N}_3 =$ \twotwomove, and
$\mathcal{N}_4 =$ \twothreemove,
We use the neighborhoods in order of their search complexity,
starting with neighborhood $\mathcal{N}_1$,
moving  to neighborhood $\mathcal{N}_{q}$, for $q=2,3,4$, only if $S$ is a 
locally optimal with respect to neighborhoods $\mathcal{N}_i$, for
$i=1,\ldots,q-1$.
That means, during the exploration of a neighborhood $\mathcal{N}_{q}$ the local search identifies all possible moves defined by the neighborhood.
As a result of an improving move, $S$ may no longer be maximal.
To deal with this issue, we iteratively add a random node with no neighbor in $S$ (from $V\setminus S$) into $S$, until the MWIS $S$ is maximal. 
Local search terminates with a solution that is locally optimal with respect
to all four neighborhoods.

There are several parameters of the local search algorithm that one can tune. First, one variation is the choice of move that the local search makes at each step. Specifically, two main approaches are 1) to identify all possible moves and choose the one that leads to the greatest gain in the objective function, and 2) search for improving moves examining potential moves in a randomized fashion and choose the first improving move that is discovered. We refer to these two approaches as best-improving selection and randomized first-improving selection, respectively. There are tradeoffs in the choice of moves at each step. For instance, the best-improving approach identifies all improving moves at each iteration, while the first-improving approach terminates the search once one improving move is discovered. In our local search implementation we use the first-improving strategy to both speed-up the running time and also increase the randomization of our method.

In Section \ref{s_local-search} we show how one can implement the local search method efficiently using customized data structures and lazy evaluation.


\subsection{Stable local optima}
\label{sec:stable-local-search}

The local search algorithm of Section \ref{sec:local-search} finds a locally optimum solution. However, some small modification outside of the local search neighborhood, may produce a better solution.
In such a case, we call the local optimum \emph{unstable}. 
Although it would be computationally expensive to test for all small perturbations to the maintained solution $S$, we use a procedure that applies random small perturbations to $S$ followed by a local search to test the stability. If the applied perturbation does not lead to a better local optimum, we retreat to the previously best local optimum. If, on the other hand, the perturbation followed by a local search leads to an improved solution, we apply future perturbations
to that solution.
If a pre-defined number of perturbation attempts fails in a row,
we stop and call the resulting locally optimal solution \emph{stable}.

Algorithm \ref{alg:stable-solution} takes as input a weighted graph $G$, an independent set $S$ of $G$ and an upper bound on the time to be spent on perturbations attempts, and outputs a stable locally optimal solution.
Three constants described below, $c_1, c_2, c_3$, tune the performance of the algorithm.
The algorithm executes two types of perturbations: {\it small} and {\it medium}.
The small perturbation $\forcerandom(S,c_1)$ selects $c_1$ nodes uniformly at random from $V \setminus S$, and forces them into $S$ by removing their neighbors from $S$. 
Every time the algorithm finds a new best local optimum, the number of small perturbations trials is set to $2*|S|+|S|/c_2$, while after every successful small perturbation (that improves the current solution but not the best one),
the number is set to $2*|S|/c_2$. 
Notice that during the perturbation we do not test whether the new independent set is better than the previous one.
To limit the divergence from the current solution,
after two consecutive iterations of small perturbations we restart the perturbation from the best local optimum found since the last medium perturbation. 
The medium perturbation $\forcerandom(S,c_3)$ is the same as the small one, but uses a parameter $c_3 > c_1$.
Our algorithm attempts small perturbations, and after a number $iter_{countdown}$ of small perturbations fail, it executes a medium perturbation. 
We repeat this for at most $i_{limit}$ time.
At the end, we return the best solution $S_{best}$  visited during the sequence of small and medium perturbations.

\begin{algorithm}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{A weighted graph, a limit $i_{limit}$ on iterations, an independent set $S$ \xspace}
	\Output{An independent set where no improving local move is possible}
	\BlankLine
	
	$S \leftarrow \LS(S)$
	
	$S_{LocOpt} \leftarrow S$;
	$S_{best} \leftarrow S$
	
	$iter_{countdown} \leftarrow 2*|S|+|S|/c_2$
	
	\For{$i_{limit}$ iterations}{
		
		$counter_{walk} \leftarrow 2$
		
		\While{$iter_{countdown} > 0$}{
			
			$counter_{walk} \leftarrow counter_{walk} - 1$
			
			\lIf{$counter_{walk}=0$}{
				$S \leftarrow S_{LocOpt}$;                
				$counter_{walk} \leftarrow 2$
			}
			
			$S \leftarrow \forcerandom(S, c_1)$
			
			$S\leftarrow \LS(S)$
			
			\uIf{$\weight{S} \geq \weight{S_{LocOpt}}$}{
				
				$S_{LocOpt} \leftarrow S$
				
				$iter_{countdown} \leftarrow 2*|S|/c_{2}$
				
				$counter_{walk} \leftarrow 2$
				
				\If{$\weight{S_{LS}} \geq \weight{S_{best}}$}{
					
					$S_{best} \leftarrow S$
					
					$iter_{countdown} \leftarrow 2*|S| + |S|/c_{2}$
				}
				
			}
			\Else{
				$iter_{countdown} \leftarrow iter_{countdown}-1$
			}
		}
		
		$S_{LocOpt} \leftarrow \LS(\forcerandom(S, c_3))$
		
		$S \leftarrow S_{LocOpt}$
		
		
	}
	Return $S$
	\caption{$\perturbLS(S_{best})$}
	\label{alg:stable-solution}
\end{algorithm}



==> s_local-search.tex <==
\section{Local Search Algorithm for MWIS}
\label{s_local-search}

Our algorithm is a metaheuristic based on a local search procedure.
We assume $S$ is an independent set. 
The neighborhood of our local search algorithm consists of the following local moves: 
\begin{itemize}
	\item \oneanymove: an improving move that adds a node $v\notin S$ to $S$ and removes any number of nodes $S_{out}\subset S$ from $S$, such that $\weight{v}>\weight{S_{out}}$.
	\item \twoonemove: an improving move that removes a node $v\in S$  from $S$ and adds two nodes $x,y \notin S$ in $S$, such that $\weight{\{x,y\}}>\weight{v}$.
	\item \twotwomove: an improving move that removes two nodes $u,v\in S$ from $S$ and adds two nodes $x,y \notin S$ to $S$, such that $\weight{\{x,y\}}>\weight{\{u,v\}}$.
	\item \twothreemove: an improving move that removes two nodes $u,v\in S$ from $S$ and adds three nodes $x,y,z \notin S$ to $S$, such that $\weight{\{x,y,z\}}>\weight{\{u,v\}}$.
\end{itemize}

We develop efficient methods for identifying each of the moves listed above. 
However, some methods require more expensive computation than other methods.
More specifically, the above list of moves appears in an increasing order of computational complexity of their search method, that is, the search of a \oneanymove move is the least expensive and the search of a \twothreemove move is the most expensive among the listed moves. 

\subsection{Supporting Data Structures}
Before describing how to efficiently identify potential moves, we introduce some data structures that will serve as the basis of our implementations.

\subsubsection*{\bf{\xmakefirstuc{\bipartitegraph.}}} Let $G=(V,E)$ be the input graph, on which the algorithm operates, and let $S$ be the independent set currently processed by the algorithm. 
Throughout the execution of the local search we maintain a graph $\mathcal{I}=(V,E_{I})$ where $E_{I}\subseteq E$ are the edges between nodes in the current independent set and those not in the independent set, i.e., $E_{I} = E \cap \{S \times \{V\setminus S\}\}$. 
%In other words, the \bipartitegraph, with respect to some independent set $S$, is a copy of $G$ where we remove all edges between nodes that are not in $S$ (notice that, by the definition of the independent set, there are no edges between nodes in $S$). 
We use the \bipartitegraph  $\mathcal{I}$  to identify the neighbors of a node $v\notin S$ that are in $S$ efficiently, i.e., $N_G(v)\cap S$, as well as the number (i.e., $|N_G(v)\cap S|$) of such neighbors of $v$.
However, as our local search algorithm transitions between neighborhoods, we need to update $\mathcal{I}$ to match the new independent set processed by the algorithm.
To maintain the \bipartitegraph efficiently after each change in $S$, we just need to update the adjacency list of the nodes that are added or removed from $S$ and their neighbors. This can be done in $O(|N_G(v)|)$ time for each node $v$ that either is added to $S$ or removed from $S$, by using hash sets to keep the adjacency lists of the nodes in $\mathcal{I}$. We maintain $\mathcal{I}$ throughout the algorithm without getting explicitly stating that it is updates.

\subsubsection*{\bf{\onetightgraph.}}  A node $w \notin S$ with a single neighbor $v$ in $S$ is called a \emph{1-tight neighbor} of $v$. A node $v\in S$ may have multiple \onetight neighbors. In our local search algorithm we wish to access efficiently the set of \onetight neighbors of a node.
Assuming $S$ is maximal, the \onetight neighbors of a node $v$ are the only nodes that can be added to $S$ if we remove only $v$ from $S$ (the rest of the nodes have at least one other neighbor in $S$ that is preventing them from being added to $S$). We maintain the \onetightgraph as follows. During the update of the \bipartitegraph $\mathcal{I}$, if the degree of a node $w\notin S$ becomes one, then we add $w$ to the \onetight neighborhood of its only neighbor. On the other hand, if the degree of a node $w\notin S$ changes from one (to either zero or two) then we remove $w$ from the \onetight neighborhood of its (previously) single neighbor. 

\subsubsection*{\bf{\twotightgraph.}}  
We call a node $w \notin S$ with exactly two neighbors $u,v$ in $S$ a \emph{2-tight neighbor} of $v$ and of $u$.
We call $v$ and $u$ \twotight mates ($v$ is a \twotight mate of $u$, and $u$ is a \twotight mate of $v$). A node $v\in S$ may have multiple \twotight neighbors.
The  {\em \twotightgraph} is a graph with a node set $V$ and two kinds of edges:
edges between the vertices in $S$ and their \twotight neighbors and edges between the pairs of \twotight mates.
We represent these edge types differently.
We maintain the edges between $w$ and its \twotight neighbors by adding the edge to the corresponding adjacency lists using hash tables to ensure constant-time additions and deletions.
To represent the edges  $(u,v)$ between \twotight mates, we maintain for each node $u\in S$ a hash map that has as a key the ID of $v$ and as a value a hash set
of the nodes $w$ that have only $u$ and $v$ as neighbors in $S$.
Whenever a node $w\notin S$ is found to have exactly two neighbors from $S$ in $G$, say the two neighbors of $w$ in $S$ are $u$ and $v$, we add the edges $\{u,w\}$, $\{v,w\}$, and $\{u,v\}$ to the \twotightgraph.
Whenever a node $w\notin S$ has no longer two neighbors from $S$ in $G$, where the two neighbors of $w$ were nodes $u$ and $v$, we remove edges $\{u,w\}$, $\{v,w\}$, and $\{u,v\}$ from the \twotightgraph.
We use the \twotightgraph in our implementation of the \twotwomove and \twothreemove procedures where we need to identify efficiently the \twotight mates of each node $v\in S$, as well as the common \twotight neighbors of $v$ with each of its \twotight mates. 


%A node $v\in S$ may have multiple \twotight neighbors and mates. In the \twotightgraph we maintain for each node $v\in S$ its \twotight mates and for each such \twotight mate $u$ of $v$ we maintain the common \twotight neighbors of $v$ and $u$.  To maintain the \twotightgraph efficiently as the set $S$ changes throughout the execution of the algorithm we proceed as follows. Whenever the degree of a node $w\notin S$ becomes exactly two, say the two neighbors of $w$ in $\mathcal{I}$ are $u$ and $v$, then we add $u$ into the set of \twotight mates of $v$ (if it is not already there) and $w$ into the set of common \twotight neighbors of $u$ and $v$. The process of adding $v$ into the data structures of $v$ is analogous. On the other hand, whenever the degree of a node $w\notin S$ changes from being equal to two, where the two neighbors of $w$ were nodes $u$ and $v$, we remove $w$ from the set of common \twotight neighbors of $u$ with $v$ and if this was the last such common \twotight neighbor we remove $v$ from the set of \twotight mates of $u$. The process of removing $u$ from the data structures of $v$ is analogous. To support efficient insertions and deletions in the set of \twotight mates and their common \twotight neighbors we maintain for each node in $v\in S$ a hash map with keys the IDs of the \twotight mates of $v$ and values hash sets with the common \twotight neighbors of $v$ and its \twotight neighbor specified by the key of the hash map. We use the \twotightgraph in our implementations of the \twotwomove and \twothreemove procedures where we need to identify efficiently the \twotight mates of each node $v\in S$, as well as the common \twotight neighbors of $v$ with each of its \twotight mates. 

\subsubsection*{\bf{Maintaining a random order of nodes in the IS}}
During the local search algorithm we process the nodes in $S$ in a random order until we find an improving move, then
continue the processing with a different random order.
A naive way to achieve this is to maintain $S$ dynamically as a hash set and to reshuffle $S$ every time we need a new random order by copying $S$ to an array and shuffling it.
However, this may lead to a significant slow-down as we spend $O(|S|)$ time to reshuffle $S$ even if we examine a small number of nodes before finding an improving mode.
To avoid this slowdown, we use lazy reshuffling.
We maintain an array $A$ with the nodes of $S$, ordered arbitrary.
In addition, we keep an array $B$ of size $|V|$ with binary values indicating whether a node is in $S$.
Let $M$ be the index of the last used location of $A$.
Whenever a node $v$ is added to $S$, we mark $B[v]$, append $v$ at the end of $A$, and increment $M$.
Whenever a node $V$ is removed from $S$, we unmark $B[v]$.
$A$ contains $S$ and potentially some elements deleted from $S$.
When we iterate over the array with the current position $i$, we first check whether the node is in $S$ and if it is not, we swap $A[i]$ it with $A[M]$, decrement $M$, and continue the iterations from position $i$.

Suppose we examined nodes in $A$ up to a position $i$.
To choose the next node to process, we pick $i \le l \le M$ uniformly at random, swap $A[l]$ with $A[i]$, and use the resulting node in $A[i]$ as the next one.


\subsection{Local Search Moves}
Next we describe efficient implementation of the local search moves.

\subsubsection*{\bf{\oneanymove}}
A naive way of finding \oneanymove moves is to iterate over all nodes $v\notin S$ and test whether $\weight{v}-\weight{N_G(v)\cap S} >0$.
If this is the case, the corresponding improving move adds $v$ to $S$ and removes $N_G(v) \cap S$ from $S$.  
However, this naive implementation requires $O(m)$. 
A faster implementation of \oneanymove maintains, for each $v\in S$, the value $\sigma(v)=\weight{v}-\weight{N_G(v)\cap S}$ dynamically as the set $S$ is updated. Whenever we remove a node $v\in S$ from $S$ we set $\sigma(w)=\sigma(w)-\weight{v}$ for all $w\in N(v)$.
Upon of an insertion of a node $v$ to $S$ we set $\sigma(w)=\sigma(w)+\weight{v}$ for all $w\in N(v)$.
Given the values $\sigma(v)$ for each node $v\notin S$, one can test in $O(n-|S|)$ time whether there exists an \oneanymove improving move.
In practice, we can speedup this computation further as we can avoid testing \oneanymove moves involving nodes $v\notin S$ whose $\sigma(v)$ value did not become positive since the last time we checked the specific move. This idea can decrease the number of nodes we need to test. However we need to maintain an updated list of nodes $v$ for which $\sigma(v)>0$. Using a hash set, this can be done in $O(1)$ time per node during the updates of the values $\sigma(v)$.

However, in practice a node can be added and removed from that list several times without being involved in a \oneanymove, and the updates are expensive because of the large constants in the use of hashing. 
We use lazy updates in the list of nodes with positive $\sigma$ value.
These updates have the same $O(1)$ amortized time but are more efficient in practice. 
Whenever the value $\sigma(v)$ of a node $v\notin S$ becomes positive and $v$ is not in the list, we add it into the list.
We implement the list using a boolean array of size $n$, for constant-time update and membership operations.
If the value  $\sigma(v)$ of a node $v\notin S$ drops becomes negative, we do not remove it from the list immediately.
Whenever we iterate through the list, we verify for each node $v$ that $\sigma(v)>0$. If this is the case, we found an improving \oneanymove move. Otherwise, we  remove $v$ from the list and proceed to the next element.
Notice that this update procedure require less time than maintaining an explicit list of the nodes with positive $\sigma$ values, as we insert a node $v$ whenever $\sigma(v)>0$, and when we identify that $\sigma(v)<0$ during the iteration over the list, we spend $O(1)$ to remove it and do not consider it again unless its $\sigma$ value becomes positive.
We gain efficiency by avoiding intermediate insertions and deletions of $v$ from the list.

\subsubsection*{\bf{\twoonemove}}
For an efficient implementation of the \twoonemove move we take advantage of the data structures that we developed. 
If $S$ is maximal, then after the removal of a node  $v\in S$ the only nodes that can be added to $S$ are the nodes whose only neighbor in $S$ is $v$.
Hence, if we remove $v$, the only candidates for insertion into $S$ are \onetight neighbors of $v$. 
Therefore, we need to identify a pair $w,z$ of non-adjacent \onetight neighbors of $v$ such that $\weight{w}+\weight{z}>\weight{v}$. 
If $v$ has $k$ 1-tight neighbors, this takes $O(k^2)$ time.\note{AVG: modified, please check}
We can further improve the running time in practice using pruning and lazy evaluation techniques.


\subsubsection*{Pruning}
For any \twoonemove that removes $v$ and adds $w,z$. we require that $\weight{w}+\weight{z}>\weight{v}$.
Therefore, if $\weight{w}+\weight{z} \leq \weight{v}$, we do not need to test
if the \onetight neighbors $w,z$ of $v$ are non-adjacent.
We use this observation as follows.
We first sort the \onetight neighbors of $v$ in descending order of their weight, and store them in an array $r$.
Next we run two nested loops, with the outer loop indexed by $i$ and the inner loop -- by $j$.
Initially $i = 1$ and $j = 2$.
When $\weight{r[i]}+\weight{r[j]}\leq\weight{v}$, we increment $i$
and restart the inner loop from position $j=i+1$.
If $2\cdot r[i] < \weight{v}$ we stop the search.

\subsubsection*{lazy evaluation}
Lazy evaluation avoids exploring combinations that we already explored in the past, they were unsuccessful, and there was no change.
If, for some node $v\in S$, $v$ acquired no new \onetight neighbor since a \twoonemove move explored $v$ the last time and failed, then we do not execute the \twoonemove moves involving $v$, as it will fail again. Notice that if \onetight neighbors is removed from the \onetight neighborhood of $v$, we also do not need to re-evaluate $v$.

We further extend the lazy evaluation idea to explore only new combinations of nodes that were not explored by the last \twoonemove move applied to $v$.
More specifically, we store the new \onetight neighbors of each node $v$ since the last time we searched all combinations of \onetight move involving $v$ and failed.
Now, if there exists an improving \onetight move involving $v$, then it must use one of the new \onetight neighbors of $v$ as all other combinations failed in the past.
Once we finish exploring all possible new pairs of \onetight neighbors of $v$, we incorporate the new \onetight neighbors of $v$ into regular \onetight neighborhood of $v$.
%\note{NP: at this point I realized that we don't have to restart with a empty regular \onetight neighborhood if $v$ is re-inserted in $S$ later, but we can still remember the failed combinations. We don't do so in the code right now}


\subsection{\twotwomove and \twothreemove}
\citet{AndResWer12a} showed, in their study of Maximum Cardinality
Independent Set problem, an algorithm to search for an \twothreemove
in $O(m\cdot \Delta)$ time. where  $\Delta$ is the maximum degree
in the graph.
The algorithm from \citet{AndResWer12a} naturally extends to weighted graphs.
We adopt the high-level search for a \twothreemove move from
\citet{AndResWer12a} and we provide an efficient implementation
using our data structures.
In order to provide an efficient search of an improving \twotwomove we use the \twotightgraph.
More specifically, we process the nodes in $S$ in a random order (to incorporate the element of randomness, to repetitively reaching the same local optima), and for each $v\in S$ that we first and for each of its \twotight mate $u$ we compute the set $C = \onetightneighbor{u} \cup \onetightneighbor{v} \cup \{\twotightneighbor{u} \cap \twotightneighbor{v}\}$ of candidate nodes for a \twotwomove move.
Finally, we test whether there exist two nodes $x,y\in C$ such that $(x,y)\notin E$ and $\weight{x}+\weight{y}>\weight{u}+\weight{v}$. 
Notice that the set $\{\twotightneighbor{u} \cap \twotightneighbor{v}\}$ are the common \twotight neighbors of $u$ and $v$, and thus, they are explicitly stored with the \twotightgraph. 
Therefore, given the \onetightgraph and the \twotightgraph we compute the set $C$ in $O(|C|)$ time.
Notice that, assuming $S$ is a maximal independent set, the set $C$ contains all possible pairs of nodes that could lead to an improving \twotwomove move replacing nodes $u,v$ as all other nodes have at least one more neighbor, other that $u$ and $v$.

The procedure for the \twothreemove moves is similar with the difference that we are looking for three common \twotight neighbors $x,y,z \in C$ of $u$ and $v$ such that $(x,y),(x,z),(y,z)\notin E$ and $\weight{x}+\weight{y}+\weight{z}>\weight{u}+\weight{v}$.


\subsubsection*{Pruning}
We apply the same idea of pruning as for the \twoonemove moves. More specifically, whenever we search for an \twotwomove removing a pair $u,v$, we first sort the nodes in $C=\onetightneighbor{u} \cup \onetightneighbor{v} \cup \{\twotightneighbor{u} \cap \twotightneighbor{v}\}$ in descending order of their weight, and store them in an array $r$.
Then, we run two iterators $i,j$ exploring all pairs $r[i],r[j]$ for which $\weight{r[i]}+\weight{r[j]}>\weight{v}+\weight{u}$ (that is, once we visit a pairs $r[i],r[j]$ that does not meet this condition we set $i = i+1$  and start the second iterator from position $j=i+1$, and if $2\cdot r[i] < \weight{v} +\weight{u}$ we stop the search).
This pruning technique aims at speeding up the search for an improving \twotwomove in practice. 

This approach trivially extends to work also for the $\twothreemove$ moves, where we run three iterators, $i,j,k$ exploring all pairs $r[i],r[j],r[k]$ for which $\weight{r[i]}+\weight{r[j]}+\weight{r[k]}>\weight{v}+\weight{u}$.

\subsubsection*{lazy evaluation}
If for some node $v\in S$ and its \twotight mate $u\in S$ there is neither a \onetight neighbor of $u$ or of $v$ nor a new common \twotight neighbor of $u$ and $v$ since the last time we searched for a \twotwomove moves removing $u$ and $v$ (and failed, otherwise $u$ and $v$ wouldn't be in $S$), then we do not have to explore set $C = \onetightneighbor{u} \cup \onetightneighbor{v} \cup \{\twotightneighbor{u} \cap \twotightneighbor{v}\}$ as the very same combinations failed the last time we search for an improving \twotwomove. Notice that if a node leaved $C$ then we still no need to re-evaluate $C$ as all remaining combinations failed in the past.

We extend the lazy evaluation idea to explore only new combinations of nodes that were not explored in the past.
More specifically, we store for each node $v\in S$ the new \onetight neighbors of $v$ and all the new common \twotight neighbors of $v$ with each of its \twotight mates since the last time we searched all combinations of \twotwomove moves involving $v$ (and failed).
Consider an improving \twotight move that results by removing $u$ and $v$.
Then, if such a move exists, then it should contain one of the new \onetight neighbors of $v$ or one of the new \onetight neighbors of $u$, or one of the new common \twotight neighbors between $u$ and $v$ as all combinations of the existing neighbors in the corresponding sets failed.
Once we explore again all possible \twotwomove moves involving $v$ and $u$, then we incorporate the new common \twotight neighbors of $v$ and $u$ into regular list of common \twotight neighborhood of $v$ and $u$.
Further, once we fail finding an improving \twotwomove move involving $v$ and any $v$'s
 \twotight mates, we incorporate the new \onetight neighborhood of $v$ into the regular \onetight neighborhood of $v$.
Notice, that the aforementioned changes in the procedure of searching for an improving \twotwomove  does not decrease the asymptotic running time, but leads to a reduced number of combinations that need to be explored. 






==> s_metaheuristic.tex <==
\section{Adoptive Path Relinking}\label{s_metaheurisitc}
In order to escape local optima, the MWIS algorithm uses a new
variant of {\em path relinking} with a randomized greedy solution~\cite{LagMar99a,RibRes12a}.
What applied to MWIS, path relinking takes the current locally optimal solution
$S^*$ and a new greedy solution $S_G$.
Then path relinking randomly orders the symmetric difference
$S^* \triangle S_G$  and  considers nodes in the symmetric difference
in this order.
We also maintain two solutions, $S'^* and S'_G$.

In our application we have $w(S^*) \gg w(S_G)$, so path relinking produces
bad solutions, and local search takes a long time to reach a new local optimum.
We modify path relinking to find a new solution such that local search from the new solution is unlikely to go back to the same local optimum and the solution quality doesn't deteriorate by too much.

The first modification is to choose the vertex $x$ to add to $S$ greedily:
we pick a vertex from $S_G - S$ to maximize the weight of the
set we get by adding $x$ to $S$ and removing its neighbors.
As a second modification, we do \emph{partial} path relinking: we stop the process after
a certain number of steps, which we adjust adaptively.
We start with a small number of steps and increase it
if the algorithm gets stuck in a local optimum of weight $w(S^*)$.

More precisely, we stop if the weight factor $f = w(S)/w(S^*)$ is smaller than a pre-defined limit, or we performed more than $c_n$ negative gain changes, or
made more than $c_p < c_n$ positive gain moves.
Positive gain moves help us escape local optima, as they will not be undone by 1-moves of the subsequent local search.
We set the initial parameter values as follows:
$f = f_0 = 0.9998$, $c_n = c_{n0} = 1.0$ and $c_p = c_{p0} = 0.1$.
If $w(S) = w(S^*)$ after local search on $S$, we multiply $f' = f \cdot 0.9998$, $c_n' = c_n \cdot 1.5$ and $c_p = c_p \cdot 1.5$.
If $w(S) \neq w(S^*)$, we reset the limits to their initial values.
If the local search algorithm finds a solution $S$ with $w(S) = w(S^*)$, we check whether the solutions are equivalent and terminate local search if they are.
Two solutions are equivalent if they are the same or if we can transform one into another by 0-gain 1-moves.


